Large Pre-trained time series models for cross-domain Time series analysis tasks

Large pre-trained models have been vital in recent advancements in domains like language and vision, making model training for individual downstream tasks more efficient and provide superior performance. However, tackling time-series analysis tasks usually involves designing and training a separate model from scratch leveraging training data and domain expertise specific to the task. We tackle a significant challenge for pre-training a foundational time-series model from multi-domain time-series datasets: extracting semantically useful tokenized inputs to the model across heterogenous time-series from different domains. We propose Large Pre-trained Time-series Models (LPTM) that introduces a novel method of adaptive segmentation that automatically identifies optimal dataset-specific segmentation strategy during pre-training. This enables LPTM to perform similar to or better than domain-specific state-of-art model when fine-tuned to different downstream time-series analysis tasks and under zero-shot settings. LPTM achieves superior forecasting and time-series classification results taking up to 40% less data and 50% less training time compared to state-of-art baselines. Code: www.github.com/AdityaLab/Samay

==> Sections/accuracy.tex <==
\clearpage
\begin{table*}[h]
	\centering
	\caption{Accuracy}
	\scalebox{0.8}{
		\begin{tabular}{|l|cccccc|}
			\hline
			                  & BasicMotions & FaceDetection & FingerMovements & PEMS-SF & RacketSports & EigenWorms \\
			\hline
			Informer          & 0.94         & 0.50          & 0.57            & 0.66    & 0.82         & 0.48       \\
			Autoformer        & 0.92         & 0.48          & 0.53            & 0.70    & 0.85         & 0.61       \\
			TimesNet          & 0.91         & 0.58          & 0.57            & 0.83    & 0.90         & 0.72       \\
			TARNet(SOTA)      & 0.99         & 0.62          & 0.61            & 0.93    & 0.97         & 0.88       \\
			TS2Vec            & 0.98         & 0.50          & 0.45            & 0.74    & 0.76         & 0.83       \\
			TS-TCC            & 0.99         & 0.53          & 0.46            & 0.72    & 0.84         & 0.76       \\
			TST               & 0.91         & 0.61          & 0.58            & 0.92    & 0.78         & 0.71       \\
			SimMTM            & 0.85         & 0.72          & 0.67            & 0.85    & 0.83         & 0.81       \\
			CRT               & 0.87         & 0.77          & 0.71            & 0.88    & 0.86         & 0.78       \\
			LPTM              & 0.99         & 0.78          & 0.77            & 0.92    & 0.92         & 0.93       \\
			LPTM-NoSegment    & 0.97         & 0.67          & 0.56            & 0.65    & 0.65         & 0.58       \\
			LPTM-NoPreTrain   & 0.95         & 0.73          & 0.61            & 0.78    & 0.78         & 0.62       \\
			LPTM-NoLinProb    & 0.99         & 0.78          & 0.68            & 0.88    & 0.92         & 0.91       \\
			LPTM-OnlyRandMask & 0.97         & 0.76          & 0.73            & 0.90    & 0.88         & 0.93       \\
			LPTM-OnlyLastMask & 0.99         & 0.75          & 0.71            & 0.86    & 0.90         & 0.88       \\
			\hline
		\end{tabular}
	}
\end{table*}

\begin{table*}[h]
	\centering
	\caption{Recall}
	\scalebox{0.8}{
		\begin{tabular}{|l|cccccc|}
			\hline
			Unnamed: 0        & BasicMotions & FaceDetection & FingerMovements & PEMS-SF & RacketSports & EigenWorms \\
			\hline
			Informer          & 0.91         & 0.49          & 0.56            & 0.64    & 0.80         & 0.47       \\
			Autoformer        & 0.89         & 0.47          & 0.52            & 0.68    & 0.82         & 0.59       \\
			TimesNet          & 0.88         & 0.57          & 0.56            & 0.81    & 0.87         & 0.70       \\
			TARNet(SOTA)      & 1.00         & 0.60          & 0.59            & 0.90    & 0.96         & 0.85       \\
			TS2Vec            & 0.98         & 0.49          & 0.44            & 0.72    & 0.74         & 0.81       \\
			TS-TCC            & 1.00         & 0.52          & 0.45            & 0.70    & 0.81         & 0.74       \\
			TST               & 0.88         & 0.59          & 0.57            & 0.89    & 0.76         & 0.69       \\
			SimMTM            & 0.82         & 0.70          & 0.65            & 0.82    & 0.81         & 0.79       \\
			CRT               & 0.84         & 0.75          & 0.69            & 0.85    & 0.83         & 0.76       \\
			LPTM              & 1.00         & 0.76          & 0.75            & 0.89    & 0.89         & 0.90       \\
			LPTM-NoSegment    & 0.96         & 0.65          & 0.55            & 0.63    & 0.63         & 0.57       \\
			LPTM-NoPreTrain   & 0.92         & 0.71          & 0.59            & 0.76    & 0.76         & 0.60       \\
			LPTM-NoLinProb    & 1.00         & 0.76          & 0.66            & 0.85    & 0.89         & 0.88       \\
			LPTM-OnlyRandMask & 0.96         & 0.74          & 0.71            & 0.87    & 0.85         & 0.90       \\
			LPTM-OnlyLastMask & 1.00         & 0.73          & 0.69            & 0.83    & 0.87         & 0.85       \\
			\hline
		\end{tabular}
	}
\end{table*}


\begin{table*}[h]
	\centering
	\caption{Precision}
	\scalebox{0.8}{
		\begin{tabular}{|l|cccccc|}
			\hline
			Unnamed: 0        & BasicMotions & FaceDetection & FingerMovements & PEMS-SF & RacketSports & EigenWorms \\
			\hline
			Informer          & 0.99         & 0.53          & 0.61            & 0.70    & 0.87         & 0.51       \\
			Autoformer        & 0.97         & 0.51          & 0.56            & 0.74    & 0.90         & 0.65       \\
			TimesNet          & 0.96         & 0.62          & 0.61            & 0.88    & 0.95         & 0.76       \\
			TARNet(SOTA)      & 1.00         & 0.66          & 0.65            & 0.98    & 1.00         & 0.93       \\
			TS2Vec            & 1.00         & 0.53          & 0.48            & 0.78    & 0.80         & 0.88       \\
			TS-TCC            & 1.00         & 0.56          & 0.49            & 0.76    & 0.89         & 0.80       \\
			TST               & 0.96         & 0.65          & 0.62            & 0.97    & 0.83         & 0.75       \\
			SimMTM            & 0.90         & 0.76          & 0.71            & 0.90    & 0.88         & 0.86       \\
			CRT               & 0.92         & 0.82          & 0.75            & 0.93    & 0.91         & 0.83       \\
			LPTM              & 1.00         & 0.83          & 0.82            & 0.97    & 0.97         & 0.98       \\
			LPTM-NoSegment    & 1.00         & 0.71          & 0.60            & 0.69    & 0.69         & 0.62       \\
			LPTM-NoPreTrain   & 1.00         & 0.77          & 0.65            & 0.83    & 0.83         & 0.66       \\
			LPTM-NoLinProb    & 1.00         & 0.83          & 0.72            & 0.93    & 0.97         & 0.96       \\
			LPTM-OnlyRandMask & 1.00         & 0.80          & 0.77            & 0.95    & 0.93         & 0.98       \\
			LPTM-OnlyLastMask & 1.00         & 0.79          & 0.75            & 0.91    & 0.95         & 0.93       \\
			\hline
		\end{tabular}
	}
\end{table*}
